Uncoupled Learning Dynamics with $O(\log T)$ Swap Regret in Multiplayer Games

In this paper we establish efficient and \emph{uncoupled} learning dynamics so that, when employed by all players in a general-sum multiplayer game, the \emph{swap regret} of each player after $T$ repetitions of the game is bounded by $O(\log T)$, improving over the prior best bounds of $O(\log^4 (T))$. At the same time, we guarantee optimal $O(\sqrt{T})$ swap regret in the adversarial regime as well. To obtain these results, our primary contribution is to show that when all players follow our dynamics with a \emph{time-invariant} learning rate, the \emph{second-order path lengths} of the dynamics up to time $T$ are bounded by $O(\log T)$, a fundamental property which could have further implications beyond near-optimally bounding the (swap) regret. Our proposed learning dynamics combine in a novel way \emph{optimistic} regularized learning with the use of \emph{self-concordant barriers}. Further, our analysis is remarkably simple, bypassing the cumbersome framework of higher-order smoothness recently developed by Daskalakis, Fishelson, and Golowich (NeurIPS'21).

==> text/bandits.tex <==
\section{Bandit Feedback Model}
\label{section:bandit}

In this section we extend our scope beyond full information feedback. Here we assume that at every iteration $t \in \N$ each player selects an action $a_i^{(t)} \sim \Vec{x}_i^{(t)}$. The most natural model one can consider is where at every iteration $t$ each player $i \in \range{n}$ only observes the \emph{realized utility} $u_i(\Vec{a}^{(t)})$ under the action profile $\Vec{a}^{(t)} = (a_1^{(t)}, \dots, a_n^{(t)})$ at round $t \in \N$. However, in this weak model even in two-player zero-sum games there is an $\Omega(\sqrt{T})$ lower bound for the sum of the players' regrets, as we formalize below.

\begin{proposition}
    \label{propsition:lb-bandit}
    Suppose that both players in a two-player zero-sum game only observe the realized utilities at every time $t \in \N$. Then, there are games for which the sum of the players' regrets is $\Omega(\sqrt{T})$. \io{More Formal}
\end{proposition}

The main observation is that there is a lower bound of $\Omega(1/\epsilon^2)$ on the support size of any $\epsilon$-approximate Nash equilibrium in zero-sum games,\io{cite}. In light of this, we consider a more benign model wherein each player $i$ observes the scalar value $u_i(a_i^{(t)}, \Vec{x}^{(t)}_{-i})$ at every time $t$. That is, the expected utility for the players' realized actions---over the randomization of the opponents. The only known result in this context is an $O(T^{1/4})$ bound on the sum of the external regrets~\citep{Wei18:More}. We substantially extend that result for the \emph{swap regret} incurred individually by each player.   
